An Experimental Study on Learning Correlated Equilibrium in Routing Games

We study route choice in a repeated routing game where an uncertain state of nature determines link latency functions, and agents receive private route recommendation. The state is sampled in an i.i.d. manner in every round from a publicly known distribution, and the recommendations are generated by a randomization policy whose mapping from the state is known publicly. In a one-shot setting, the agents are said to obey recommendation if it gives the smallest travel time in a posteriori expectation. A plausible extension to repeated setting is that the likelihood of following recommendation in a round is related to regret from previous rounds. If the regret is of satisficing type with respect to a default choice and is averaged over past rounds and over all agents, then the asymptotic outcome under an obedient recommendation policy coincides with the one-shot outcome. We report findings from an experiment with one participant at a time engaged in repeated route choice decision on computer. In every round, the participant is shown travel time distribution for each route, a route recommendation generated by an obedient policy, and a rating suggestive of average experience of previous participants with the quality of recommendation. Upon entering route choice, the actual travel times are revealed. The participant evaluates the quality of recommendation by submitting a review. This is combined with historical reviews to update rating for the next round. Data analysis from 33 participants each with 100 rounds suggests moderate negative correlation between the display rating and the average regret, and a strong positive correlation between the rating and the likelihood of following recommendation. Overall, under obedient recommendation policy, the rating converges close to its maximum value by the end of the experiments in conjunction with very high frequency of following recommendations.

==> An Experimental Study on Learning Correlated Equilibrium in Routing Games/abstract-ks.tex <==
\begin{abstract}
We study route choice in a repeated routing game where an uncertain state of nature determines link latency functions, and the agents receive private route recommendation. The state is sampled in an i.i.d. manner in every round from a publicly known distribution, and the recommendations are generated by a randomization policy whose mapping from the state is also known publicly. In a one-shot setting, the agents are said to \emph{obey} recommendation if it gives the smallest travel time in a posteriori expectation. A plausible extension to repeated setting is that the likelihood of following recommendation in a round is related to \emph{regret} from previous rounds. If the regret is of satisficing type with respect to a default choice and is averaged over past rounds and over all agents, then the asymptotic outcome under an obedient recommendation policy is known to coincide with the one-shot outcome. We report findings from a related experiment with one participant at a time engaged in repeated route choice decision on computer. In every round, the participant is shown travel time distribution for each route, a route recommendation generated by an obedient policy, and a numeric rating suggestive of average experience of previous participants with the quality of recommendation. Upon entering route choice, the actual travel times derived from route choice of previous participants are revealed. The participant uses this information to evaluate the quality of recommendation received for that round and enter a numeric review accordingly. This is combined with historical reviews to update rating for the next round. Data analysis from 33 participants each with 100 rounds suggests moderate negative correlation between the display rating and the average regret with respect to optimal choice, and a strong positive correlation between the rating and the likelihood of following recommendation. Overall, under obedient recommendation policy, the rating seems to converge close to its maximum value by the end of the experiments in conjunction with very high frequency of following recommendations. 
%has identified sufficient conditions for convergence. In this paper, we report findings from an experimental study inspired by the theoretical setup. The atomic setup is approximated by an atomic setup with a single human participant and a continuum of automated participants whose decisions and review is derived from past participants. Experimental findings show strong correlation between xyz and xyz and a medium correlation between xyz and xyz. 


%The purpose of this study is to understand drivers' route choice decision-making patterns in traffic networks with travel time uncertainties when route recommendations are provided by platforms. We study drivers' long-term compliance behavior so that route recommendation platforms can better persuade drivers to follow the recommendations while minimizing the expected social travel time. Study participants will click through a number of traffic network scenarios on a computer interface and make route choice decisions based on route recommendations, the average star rating and the spread of travel times. They are asked to rate recommendations upon completion of each scenario. We show that, if the route recommendation strategy adopted by the platform satisfies a certain obedience property, then the agents' compliance rate will become 100\% in the long run. 
\end{abstract}

==> An Experimental Study on Learning Correlated Equilibrium in Routing Games/acknowledgment-ks.tex <==
\section*{Acknowledgment}
The authors thank Christine Stavish for help with writing code for the experiment interface and for setting up data management. The authors also thank Christine Stavish, Grace Foltz, and Alejandra Reyes for help with conducting the experiments. 

==> An Experimental Study on Learning Correlated Equilibrium in Routing Games/background-ks.tex <==
\section{Theoretical Background}
\label{sec:theory}
We start by providing summarizing model and results from our previous work in \cite{Zhu.Savla:DGAA21} which forms the basis of hypotheses to be tested in the experiments. 

Consider a network consisting of $\nlinks$ parallel links between a single source-destination pair. Without loss of generality, let the agent population generate a unit volume of traffic demand. The link latency functions $\congfunc_{\omega,i}(f_i)$, $i \in [\nlinks]$, give latency on link $i$ as a function of flow $f_i$ through them, conditional on the \emph{state} of the network $\state \in \allstates=\{\state_1, \ldots,\state_{|\Omega|}\}$. The latency function is in the following form:
\begin{equation}
\label{eq:polynomial-latency-function}
\congfunc_{\omega,i}(f_i) =  \sum^D_{d=0} \alpha_{d,\omega,i} \, f_i^d, \, i \in [\nlinks], \, \, \state \in \allstates
\end{equation}
Let $\state \sim \prior \in \interior(\triangle(\allstates))$, for some prior $\prior$ which is known to all the agents. The agents do not have access to the realization of $\state$, but a fixed fraction $\pfrac \in [0,1]$ of the agents receives private route recommendations conditional on the realized state (in the experiments, we have $\nu = 1$, i.e. all agents reveive recommendations). These conditional recommendations are generated by a \emph{diagonal atomic signal} $\signal=\{\signal_{\state} \in \simplex_{\nlinks}: \, \state \in \allstates\}$~\cite{Zhu.Savla:TCNS22}.

Consider the following repeated game setting. The strategy space of  every agent is $\{\mathrm{follow}, \mathrm{do \, not \, follow}\}$. The $\mathrm{do \, not \, follow}$ behavior of the agents is modeled by the row-stochastic matrix $P$ with zeros on the diagonal, where $P_{ij}$ is the fraction of $\mathrm{do \, not \, follow }$ agents who are recommended $i$ but choose $j$. The choice of a agent is driven by a notion of regret. At the end of stage $k$, every agent computes difference between the payoffs associated with the default choice and the recommended choice. These payoff differences are then aggregated over the entire agent population to give $u(k)$. The average of the initial condition $m(1)$ and $u(1), \ldots, u(k)$, denoted as $m(k+1)$, is then mapped to regret as $\theta(m(k+1)) \in [0,1]$, which equals the fraction of agents who do not follow recommendation in stage $k+1$. The details for each step in this process is provided next. 

We assume that upon completion of the trips, all the agents have access to traffic report from the $k$-th stage. This report consists of $\omega(k)$ and $\{\ell_{\omega(k),i}\}_{i \in [n]}$. For simplicity, first consider the two-link case with $\ell_{\omega(k),1}>\ell_{\omega(k),2}$. For an agent who was recommended route 1, irrespective of whether she follows the recommendation or not, her recommendation is sub-optimal by $\ell_{\omega(k),1}-\ell_{\omega(k),2}$. In the general case of $n \geq 2$ links, for an agent who follows recommendation to take route $i$, the sub-optimality of the recommendation is $\congfunc_{\omega(k),i} -\sum_{j \in [n]} P_{ij} \congfunc_{\omega(k),j}$. On the other hand, for an agent who does not follow the recommendation to take route $i$ but rather takes route $j$, the sub-optimality of her recommendation is $\congfunc_{\omega(k),i} -\congfunc_{\omega(k),j}$. Taking into account the number of agents who are recommended different routes and the fraction of them who $\mathrm{follow}$ or $\mathrm{do \, not \, follow}$ the recommendation, the aggregation of payoff difference over the entire agent population is given by:
\begin{align}
u(k) := & \sum_{i \in [n]} \Big(\congfunc_{\omega,i} -\sum_{j \in [n]} P_{ij} \congfunc_{\omega,j} \Big) \pi_{\omega,i} \left(1-\theta(m(k))\right) + \sum_{i,j \in [n]} \Big(\congfunc_{\omega,i} - \congfunc_{\omega,j} \Big) P_{ij}\pi_{\omega,i} \theta(m(k)) \nonumber \\
=& \sum_{i,j \in [n]} \Big(\congfunc_{\omega,i} - \congfunc_{\omega,j} \Big) P_{ij} \pi_{\omega,i} 
= {\pi_{\omega}}^T (I-P) \congfunc_{\omega}
\label{eq:instant} 
\end{align}
where we have dropped the dependence of $\{\ell_{\omega,i}\}_{i \in [n]}$, $\{\pi_{\omega,i}\}_{i \in [n]}$ and $\omega$ on $k$ for brevity. 
%In the spirit of transparency, we assume that the the structure of the dynamics in \eqref{eq:S-agent-update} is known to the B-agents. 
The average of these instantaneous payoff differences (as well as the initial condition $m(1)$) is:
\begin{equation}
\label{eq:S-agent-update}
\begin{split}
m(k+1) & = \frac{1}{k+1} \left(m(1)+ u(1) + \ldots u(k) \right) = \frac{k}{k+1} m(k) + \frac{1}{k+1} u(k)
\end{split}
\end{equation}

We adopt the following notion of regret:
\begin{equation}
\label{eq:rating-to-mistrust}
\theta(m(k))=\frac{[m(k)]^+}{m_{\max}}
\end{equation}
where $m_{\max}$ is chosen to be sufficiently large so that $\theta(m(k)) \in [0,1]$ for all possible values of $m(k)$. Since $[m(k)]^+$ can be upper bounded by $\sum_{i \in [n]} \sum_{ d=0}^D \max_{\omega \in \Omega} \alpha_{d,\omega,i}$, it can then serve as a lower bound for $m_{\max}$.

$\theta(m(k))$ is interpreted as the fraction of agents who do not follow recommendation. 
Therefore, the link flows induced by the agents is given by: \ksmarginphantom{need more details for \eqref{eq:p flow dynamics-m-general}}
\begin{equation*}
\label{eq:p flow dynamics-m-general}
\begin{split}
f_i(m(k),\omega(k)) = \pi_{\omega(k),i} \left(1-\theta(m(k))\right) + \sum_{j \in [n]} P_{ji} \pi_{\omega(k),j} \theta(m(k))
\end{split}
\end{equation*}
which in matrix form becomes:
\begin{align}
%\label{eq:p flow dynamics-m-general-matrix}
%\begin{split}
f(m(k),\omega(k)) & = \pi_{\omega(k)} \left(1-\theta(m(k))\right) + \sum_{j \in [n]} P_{ji} \pi_{\omega(k),j} \theta(m(k)) = \pi_{\omega(k)} - \theta(m(k)) \pi_{\omega(k)} + \theta(m(k)) P^T \pi_{\omega(k)}  \nonumber \\
& = \pi_{\omega(k)} + \theta(m(k)) (P^T - I ) \pi_{\omega(k)}
\label{eq:p flow dynamics-m-general-matrix}
%\end{split}
\end{align}

\begin{remark}
The framework in \eqref{eq:instant}-\eqref{eq:p flow dynamics-m-general-matrix} is reminiscent of the \emph{regret matching} framework of \cite{Hart.Mas-Colell:00}. A few points are worth special emphasis:
\begin{enumerate}
\item The aggregation of payoff difference over all agents in \eqref{eq:instant} is inspired by platforms such as Yelp. 
\item In the framework of \cite{Hart.Mas-Colell:00}, $[m]^+$ is referred to as regret and $m_{\max}$ is the inertia parameter which captures the propensity of an agent to stick to the action choice in the previous round. On the other hand, in our setup, $\theta=[m]^+/m_{\max}$ is interpreted as the degree of obedience of an individual agent, tuned by the parameter $m_{\max}$.
\end{enumerate}
\end{remark}

We consider $\signal$ which are \emph{obedient}, i.e., which satisfy
%to the \emph{Bayes Correlated Equilibrium}~\cite{Bergemann.Morris:16} induced by $\signal$, i.e., $(\signal,y \in \simplex_{\nlinks}(1-\pfrac))$ satisfying the following:
%\begin{equation}
$\sum_{\state} \ell_{\omega,i}(\signal_{\state,i}) \, \signal_{\state,i} \, \prior(\state) \leq \sum_{\state}  \ell_{\omega,j}(\signal_{\state,j}) \, \signal_{\state,i} \, \prior(\state)$ for all $i, j \in [\npaths]$. We showed in \cite{Zhu.Savla:DGAA21} that, for any $\prb$, obedient $\pi$, and every $m(1) \in [-m_{\max},+m_{\max}]$, the solution to \eqref{eq:instant}-\eqref{eq:p flow dynamics-m-general-matrix} satisfies $\lim_{k \rightarrow \infty} f_i(k) - \pi_{\omega(k),i} = 0$ for all $i \in [n]$.


==> An Experimental Study on Learning Correlated Equilibrium in Routing Games/conclusion-ks.tex <==
\section{Conclusion and Future Work}
\label{sec:conclusion}
%\kscomment{
%Discussion:
%\begin{itemize}
%\item Strong justification for several modeling choices in theoretical analysis
%\item Long run convergence of display rating, and also frequency of recommendation following. This was the main objective. However, we also get justification for our model for repeated setting. In particular, 
%Strong correlation between display and likelihood of following. 
%(Does review by participants also converge to a high value in the long run?)
%\item Notion of regret still needs more work; concrete directions to pursue for theoretical analysis
%\item First experimental study on information design for multi round setting. Probably first on convergence to a specific correlated equilibrium. 
%\end{itemize}
%}
%
The immediate utility of the proposed experimental setup is to provide a setting which induces high rate of following of private route recommendation in traffic networks with uncertain travel times. The fact that the experiment design mirrors setup for a learning model with provable convergence to the Bayes correlated equilibrium induced by the obedient policy in our prior work in \cite{Zhu.Savla:DGAA21} gives further credence to this setting. In addition to providing evidence for overall convergence, our analysis also provides insight into empirical validity of key components of the learning model. Specifically, we found strong correlation between the likelihood of a particular agent following recommendation with the summary statistic of experience of other agents encapsulated by the displayed rating. The empirical route choice distributions conditional on recommendation also seem to converge. The fact that we found only moderate correlation in general between the average regret and the displayed rating, and that several participants self-reported to follow the recommendation even for medium values of displayed rating suggests further investigation is needed to conclusively establish regret as a key driver in learning. Our experimental strategy to approximate non-atomic games with atomic settings could be of independent interest for experimental studies in non-atomic games, especially with regards to correlated equilibria.  

Directions for testing robustness of the experimental findings reported in this paper include randomizing initial condition on display rating for participants as well as the default value on the slider used for collecting review from the participants, and relaxing explicit suggestions to the participants for following a specific route choice strategy. It would also be interesting to repeat the experiments under an obedient policy which induces a \emph{bad} correlated equilibrium~\cite{Duffy2010}, i.e., which is (Pareto) inferior to the Bayes Wardrop equilibrium. 
%The experimental findings provide several interesting directions for theoretical modeling and analysis on convergence to correlated equilibria. On one hand, there is no clear validity of the usual notions of regret as drivers of decision, but on the other hand, the feedback survey provides a collection of self-reported strategies. Expanding the scale of the experiments to more participants could provide insights into emergence of dominant clusters of such self-reported strategies. 
It would also be interesting to explore connection between our agent model in \eqref{eq:instant}-\eqref{eq:p flow dynamics-m-general-matrix} and the learning models in \cite{Arifovic.Ledyard:11,Arifovic.Boitnott.ea:19}.   


==> An Experimental Study on Learning Correlated Equilibrium in Routing Games/config-ks.tex <==
\pdfminorversion=4
\usepackage{amsmath,amssymb,bbm,color,psfrag,amsfonts,mathtools}
\usepackage{dsfont}
\usepackage{graphicx,cuted}                       % \includegraphics
%\usepackage[normalem]{ulem}    
\usepackage[pdftex,pdfpagelabels,bookmarks,hyperindex,hyperfigures]{hyperref}
\usepackage{wrapfig}
\usepackage{pdfpages}
\usepackage[ruled,lined]{algorithm2e} 
\usepackage{algpseudocode}% http://ctan.org/pkg/algorithmicx
%\usepackage{algorithm}% http://ctan.org/pkg/algorithm
   \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
\usepackage{accents}
\usepackage{lipsum}
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
\usepackage{mathtools}
\usepackage{multicol}
\usepackage{paralist}   % \begin{inparaenum}[1)]
\usepackage{comment}
\usepackage{kbordermatrix}
\usepackage{tikz}

%\usepackage{enumitem}
%\setlist{parsep=0pt,listparindent=\parindent}

% revision mode 
%\usepackage{changes}
%\definechangesauthor[name={Qin}, color=orange]{q}
%\setremarkmarkup{(#2)}

% table
\usepackage{booktabs}  
\usepackage{multirow}
\usepackage[normalem]{ulem}

% caption
\usepackage{caption}
\captionsetup{width=1.0\columnwidth}
\usepackage{subcaption}

\usepackage{cite}


% algorithm
%\usepackage{algorithmic}
%\usepackage{algorithm}
% theorem environment. 
%\theoremstyle{plain} 

%\newenvironment{problem}[1][htb]
%  {\renewcommand{\algorithmcfname}{Problem}% Update algorithm name
%   \begin{algorithm}[#1]%
%  }{\end{algorithm}}

\newcounter{problem}
\newenvironment{problem}[1][]
{\refstepcounter{problem} \medskip 
\noindent
\begin{tabular}{@{}p{\textwidth}} 
\\ \toprule 
 \textbf{Problem~\theproblem:}  #1 
   \\  \midrule
   }
   {\vspace{-0.6cm} \\ \bottomrule \end{tabular}  \medskip}


\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{conjecture}{Conjecture}
\newtheorem{hypothesis}{Hypothesis}
\newtheorem{result}{Result}

%\theoremstyle{definition}
\newtheorem{definition}{Definition}
\newtheorem{assumption}{Assumption}

%\theoremstyle{remark}
\newtheorem{remark}{Remark}
\newtheorem{example}{Example}

% QED filled black box

%%% Annotation
\usepackage{color}

%% new commands

\newcommand{\ubar}[1]{\underaccent{\bar}{#1}}

% frequently used sets
\newcommand{\ones}{\mathbf 1}
%\newcommand{\real}{{\mbox{\bf R}}}
\newcommand{\real}{\mathbb{R}}
\newcommand{\complex}{\mathbb{C}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\mc}{\mathcal}
\newcommand{\kscomment}[1]{{\color{red} #1}}
\newcommand{\yzcomment}[1]{{\color{blue} #1}}
%\newcommand{\kscomment}[1]{#1}
%\newcommand{\kscommentphantom}[1]{{\color{red} #1}}
\newcommand{\kscommentphantom}[1]{#1}
\newcommand{\kscommentcancel}[1]{{\color{red} #1}}
\newcommand{\ksmargin}[1]{\marginpar{\color{red}\footnotesize [KS]:
#1}}
\newcommand{\yzmargin}[1]{\marginpar{\color{blue}\footnotesize [YZ]:
#1}}
\newcommand{\ksmarginphantom}[1]{}
\newcommand{\yzmarginphantom}[1]{}

\newcommand{\argmin}{\mathop{\rm argmin}}
\newcommand{\argmax}{\mathop{\rm argmax}}
\newcommand{\setdef}[2]{\left\{#1 \; | \; #2\right\}}
\newcommand{\zerobf}{\mathbf{0}}
\newcommand{\onebf}{\mathbf{1}}
\newcommand{\until}[1]{\{1,\dots,#1\}}
\newcommand{\map}[3]{#1: #2 \rightarrow #3}
\newcommand{\ds}{\displaystyle}

\newcommand{\fr}{\nu}
\newcommand{\prb}{\mu_0}
\newcommand{\cost}{J}
\newcommand{\congfunc}{\ell}
\newcommand{\diag}{\mathbf{diag}}

\newcommand{\prior}{\mu_0}
\newcommand{\state}{\omega}
\newcommand{\allstates}{\Omega}
\newcommand{\interior}{\mathrm{int}}
\newcommand{\signal}{\pi}
\newcommand{\signalmarginal}{{\overline{\signal}}}
\newcommand{\pfrac}{\nu}
\newcommand{\simplex}{\mc P}
\newcommand{\supersimplex}{\mathbf{P}}
\newcommand{\nlinks}{n}
\newcommand{\npaths}{\nlinks}
\newcommand{\nmesgs}{m}
\newcommand{\nsup}{r}
\newcommand{\nstates}{s}
\newcommand{\E}{\mathbb{E}}
\newcommand{\posterior}{\mu}
\newcommand{\pflowfull}{f^{P,\text{full}}}
\newcommand{\bwe}{\mc B}
\newcommand{\allcongfunc}{\mc L}
\newcommand{\congfuncallstates}{L}
\newcommand{\allsignals}{\Pi}
\newcommand{\allpubsignals}{\Pi^{\text{pub}}}
\newcommand{\allsignalsposterior}{\hat{\Pi}}
\newcommand{\vect}{\mathrm{vec}}
\newcommand{\supp}{\mathrm{supp}}
\newcommand{\avgcongfunc}{\bar{\congfunc}}
\newcommand{\messagespace}{\mc M}
\newcommand{\rowstochastic}{\mc R}
\newcommand{\powerset}{\mathbb{P}}
\newcommand{\regret}{r}
\newcommand{\regretplain}{I}
\newcommand{\instregret}{I^{\text{inst}}}
\newcommand{\avgregret}{I^{\text{avg}}}
\newcommand{\regretmax}{I_{\max}}
\newcommand{\regretpub}{r^{\text{pub}}}
\newcommand{\pagentprob}{p}
\newcommand{\defprob}{q^{\text{def}}}
\newcommand{\defprobtwo}[2]{\defprob_{#1,#2}}
\newcommand{\actprob}[2]{\actprobplain_{#1,#2}}
\newcommand{\de}{\mathrm{d}}
\newcommand{\pubsignal}{\signal^{\text{pub}}}
\newcommand{\sender}{\mathbb{S}}

\newcommand{\multmu}{p}
\newcommand{\multlambda}{q}
\newcommand{\mom}{\eta}

\newcommand{\sgn}{\mathrm{sgn}}
\newcommand{\degree}{\mathrm{deg}}
\newcommand{\rank}{\mathrm{rank}}

\newcommand{\numsubjects}{S}
\newcommand{\numscenarios}{K}
\newcommand{\Rmax}{r_{\max}}

\graphicspath{{../},{../results/} , {../../../../fig/},{../fig/}}
%\graphicspath{{../../../fig/}}

\algnewcommand{\algorithmicgoto}{\textbf{go to}}%
\algnewcommand{\Goto}[1]{\algorithmicgoto~\ref{#1}}%

\setcounter{MaxMatrixCols}{20}




==> An Experimental Study on Learning Correlated Equilibrium in Routing Games/extra-stuff-ks.tex <==
\subsection{Extra Stuff}
We now describe the modifications to the model in \eqref{eq:instant}-\eqref{eq:p flow dynamics-m-general-matrix} to align it with the experimental setup. 
\begin{itemize}
\item Recall from \eqref{eq:instant}-\eqref{eq:p flow dynamics-m-general-matrix}  that matrix $P$ is used in the computation of regret. Since we do not know $P$ a priori, we replace it with the following online estimate for the $s$-th agent:
\begin{equation*}
\hat{P}_{i,j}^{s}= \frac{N(s-1;i,j)}{\sum_{j \in (\nlinks)} N(s-1;i,j)}, \quad i, j \in (\nlinks)
\end{equation*}
where $N(s-1;i,j)$ is the number of times agents $1$ thru $s-1$ choose route $j$ when recommended route $i$. That is, $\hat{P}^{s}$ is constant during session of agent $s$.

\item At the beginning of scenario $k$, participant $\#n$ checks the average review rating $R^{\#n}[k]$ (maximum 5 star rating), combines with the recommended route and the histograms, participant $\#n$ makes his or her route choice decision. Irrespective of participant $\#n$'s decision, the route flow on route $i, i \in (3)$ is given by: 
\begin{equation*}
\label{eq:p flow dynamics-m-general}
\begin{split}
f_i(R^{\#n}[k],\omega[k]) = \pi_i^{\omega[k]} \frac{R^{\#n}[k]}{5} + \sum_{j \in (3)} P^{\#n}_{ji} \pi_j^{\omega[k]} \left(1-\frac{R^{\#n}[k]}{5}\right)
\end{split}
\end{equation*}


\item We mimic the simultaneous routing behavior of multiple participants by incorporating submitted review ratings of all past participants, under the same realized state of nature $\omega[k]$ and the same quantized average review rating $\tilde{R}^{\#n}[k]$ (quantization step = 0.5), when updating the average review rating $R^{\#n}[k+1]$ after participant $\#n$ submitted his or her review rating $r^{\#n}[k]$. Let $\mc R^{\#n}_{\omega[k],\tilde{R}^{\#n}[k]}:=\{r^{\#h}[t] | h \in (n), \omega[t]=\omega[k], \tilde{R}^{\#h}[t]=\tilde{R}^{\#n}[k]\}$, the instantaneous aggregated rating is given by:
\begin{equation*}
\bar{r}^{\#n}[k] := \frac{\sum_{r^{\#h}[t] \in \mc R^{\#n}_{\omega[k],\tilde{R}^{\#n}[k]}} r^{\#h}[t]}{\left|\mc R^{\#n}_{\omega[k],\tilde{R}^{\#n}[k]}\right|}
\end{equation*}
The average review rating of scenario $k+1$ for participant $\#n$ is given by:
\begin{equation*}
R^{\#n}[k+1]=\frac{k}{k+1}R^{\#n}[k]+\frac{1}{k+1}\bar{r}^{\#n}[k]
\end{equation*}
Then, participant $\#n$ will enter scenario $k+1$ with the updated average review rating $R^{\#n}[k+1]$, untill $k=100$ and the experiment session will end for participant $\#n$. 
\end{itemize}


%\subsection{Repeated Game Setting}
%Consider the following repeated game setting. The strategy space of a participant is $\{\mathrm{obey}, \mathrm{do \, not \, obey}\}$. The $\mathrm{do \, not \, obey}$ behavior of the participant is modeled by the row-stochastic matrix $P$ with zeros on the diagonal, where $P_{ij}$ is the fraction of $\mathrm{do \, not \, obey }$ participants who are recommended route $i$ but choose $j$. 
%
%In the experiment study, we use the route choice data from participant $\#1$ up to $\#n-1$ to calculate $P^{\#n}$ for participant $\#n$. For example, $P^{\#n}_{ij} := \frac{\text{total number of times of choosing route j when recommended route i for participants \#1 up to \#n-1}}{\text{total number of times of not following the recommendation when recommended route i for participants \#1 up to \#n-1}}$. 

After making his or her route choice for scenario $k$, participant $\#n$ will then have access to realized actual travel times $\{\ell_i^{\omega[k]}\}_{i \in (3)}$, and be asked to evaluate the quality of the recommendation and submit a rating $r^{\#n}[k]$. 

\ksmargin{move it to later?}
\kscomment{Note that, we set the initial values of average review rating $R^{\#n}[1]$ for all participants $n$ to be 2.5.}

In our theoretical work, the choice of a participant is driven by a notion of regret. To study the relation between instantaneous aggregated average rating and regret, we have to define regret properly. In our theoretical work, the regret model requires knowledge of $P$, which can only be computed using historical data of all previous participants and is inaccessible to the current participants. Based on the available information in our user interface, which consists of actual travel times of all 3 routes, we redefined the individual regret as the difference between the actual travel time of recommended route and fastest route.

After making his or her route choice for scenario $k$, participant $\#n$ will then have access to realized actual travel times $\{\ell_i^{\omega[k]}\}_{i \in (3)}$, and compute the instantaneous regret $m^{\#n}[k]$ as the difference between the travel time associated with the recommended route and the shortest travel time. Similar to the aggregation mechanism of instantaneous aggregated rating, we incorporate instantaneous regrets of all past participants, under the same realized state of nature $\omega[k]$ and the same quantized average review rating $\tilde{R}^{\#n}[k]$ (quantization step = 0.5), when calculating the instantaneous aggregated regret $\bar{m}^{\#n}[k]$. Let $\mc M^{\#n}_{\omega[k],\tilde{R}^{\#n}[k]}:=\{m^{\#h}[t] | h \in (n), \omega[t]=\omega[k], \tilde{R}^{\#h}[t]=\tilde{R}^{\#n}[k]\}$, the instantaneous aggregated regret is given by:
\begin{equation*}
\bar{m}^{\#n}[k] := \frac{\sum_{m^{\#h}[t] \in \mc M^{\#n}_{\omega[k],\tilde{R}^{\#n}[k]}} m^{\#h}[t]}{\left|\mc M^{\#n}_{\omega[k],\tilde{R}^{\#n}[k]}\right|}
\end{equation*}
And the time-averaged aggregated regret is given by:
\begin{equation*}
\tilde{m}^{\#n}[k] := \frac{1}{k} \sum_{t=1}^k \bar{m}^{\#n}[t]
\end{equation*}

==> An Experimental Study on Learning Correlated Equilibrium in Routing Games/fig/block-diagram.tex <==
\begin{tikzpicture}
\draw[very thick] (-1.85,-0.5) -- (-1.85,0.5) -- (1.85,0.5) -- (1.85,-0.5) -- (-1.85,-0.5);
\draw (0,0) node {\Large participant $s$};
%\draw (0,-0.2) node {\Large $s$};

\draw[very thick] (-1.25,-2.5) -- (-1.25,-1.5) -- (1.25,-1.5) -- (1.25,-2.5) -- (-1.25,-2.5);
\draw (0,-2) node {\Large Eq. \eqref{eq:subject-model}};

\draw[very thick] (-1.25,2.5) -- (-1.25,1.5) -- (1.25,1.5) -- (1.25,2.5) -- (-1.25,2.5);
\draw (0,2) node {\Large Eq. \eqref{eq:human-output-to-input-1} \eqref{eq:human-output-to-input-2}};
\draw (3.5,-2.25) node {\large $\hat{m}^s$};

\draw (-3.5,2.25) node {\large route recommendation $i$};
\draw (-2,1.7) node {\large $(f^s,r^s)$};

\draw[very thick,->] (1.85,0) -- (3.15,0);
\draw[very thick,->] (1.25,-2.25) -- (3.15,-2.25);

\draw[very thick] (2.25,0) -- (2.25,-1.75);
\draw[very thick,->] (2.25,-1.75) -- (1.25,-1.75);

\draw[very thick] (2.25,0) -- (2.25,2.0);
\draw[very thick,->] (2.25,2.0) -- (1.25,2.0);

\draw[very thick] (-1.25,2.0) -- (-2.75,2.0) -- (-2.75,-1.75);
\draw[very thick,->] (-2.75,0) -- (-1.85,0);
\draw[very thick,->] (-2.75,-1.75) -- (-1.25,-1.75);

\draw (3.75,0.3) node {\large route choice $j$};
\draw (3.25,-0.3) node {\large review};

\end{tikzpicture}

==> An Experimental Study on Learning Correlated Equilibrium in Routing Games/findings-ks.tex <==
\section{Experiment Findings}
\label{sec:findings}
\subsection{Experiment Parameters}
The parameters in our experiments were $\nlinks=3$, $|\Omega|=5$,  
$\numsubjects=33$\footnote{34 participants were recruited in total, but one participant faced technical error during experiment, and therefore we discarded the data from this participant from our analysis.}, $\numscenarios=100$, $\hat{P}^1=\begin{bmatrix}0&0&1\\0&0&1\\0.5&0.5&0\end{bmatrix}$, $r^s(1)=2.5$ for all $s \in [\numsubjects]$, $\Rmax=5$, 
%
%
%\subsection{Non-atomic Routing Game with Signaling}
%Since the participants will participate sequentially, we make some changes to the theoretical model to mimic the simultaneous routing behavior of multiple participants. We consider a network consisting of $3$ parallel links between a single source-destination pair. Without loss of generality, let there be a unit volume of traffic demand. Due to the non-atomic population model we are using, a single participant's routing decision will not affect the realized travel times. The link latency functions $\congfunc_{i}^{\omega}(f_i)$, $i \in (3)$, give travel time on link $i$ as a function of flow $f_i$ through them, conditional on the \emph{state} of the network $\state \in \allstates=\{\state_1, \ldots,\state_5\}$. In this experimental study, we restrict ourselves to affine latency function in the form of $\congfunc_{i}^{\omega}(f_i) =  \alpha_{0,i}^{\omega} + \alpha_{1,i}^{\omega} \, f_i$. Specifically, we choose the following parameters for the experiment study: 
\begin{equation*}
\alpha_0 = 
\kbordermatrix{&i=1&i=2&i=3\\
\omega_1&5&25&4\\
\omega_2&20&15&24\\
\omega_3&15&20&14\\
\omega_4&11&15&16\\
\omega_5&8&10&20}, \quad 
\alpha_1 = 
\kbordermatrix{&i=1&i=2&i=3\\
\omega_1&4&2&1\\
\omega_2&1&2&3\\
\omega_3&2&3&4\\
\omega_4&3&5&2\\
\omega_5&5&4&5}, \quad
\pi = 
\kbordermatrix{&i=1&i=2&i=3\\
\omega_1&0.1&0&0.9\\
\omega_2&0&1&0\\
\omega_3&0.6&0&0.4\\
\omega_4&0.9&0.1&0\\
\omega_5&0.6&0.4&0}
\end{equation*} \ksmarginphantom{need to rather compare link-wise travel times under policy and Wardrop}
The $\pi$ chosen is an optimal solution to the \emph{information design problem}~\cite{Zhu.Savla:TCNS22}, i.e., it minimizes social cost among all obedient policies. Indeed, the social cost under this policy is about 13\% lower than under Bayes Wardrop equilibrium. 
The sequence $\{\omega(k)\}_{k=1}^{100}$ is sampled offline in an i.i.d. manner from $\mu_0=[0.1 \, \, 0.2 \, \, 0.4 \, \, 0.05 \, \, 0.25]$. The empirical distribution of the sampled sequence is equal to the prior $\mu_0$, and the same sampled sequence is used for all the participants. 
 
%A total of 34 participants were recruited. Each participant completed 100 scenarios, with one exception for participant $\#7$ when an error occurred and only 9 scenarios were completed before the session was ended intentionally to recover from the error. After eliminating those 9 faulty scenarios of participant $\#7$, we collected data of 3300 useable scenarios overall. 

\subsection{Recommendation Following vs Displayed Rating}
\label{sec:hypo1}
\begin{figure}[htb!]
\begin{center}
\begin{minipage}[c]{.475\textwidth}
\begin{center}
\includegraphics[width=1.0\textwidth]{hypo1} 
\end{center}
\end{minipage}
\end{center}
\caption{\sf Linear regression between empirical probability of recommendation and quantized displayed rating.}
\label{fig:hypo1}
\end{figure}
For the sake of analysis, we quantized the displayed rating by rounding off to one decimal place. We computed empirical probabilities of following recommendation over all participants and all scenarios for each quantized displayed rating. We discarded data associated with the displayed rating interval $[2.6,3.9]$ because the rating changed so rapidly in $[2.6,3.9]$ that the  participants saw a specific display rating in the range $[2.6,3.9]$ for less than one scenario on average. Given such a low sample size, the statistics for following recommendation conditional on display rating in the interval $[2.6,3.9]$ would not be reliable. Moreover, these discarded data points accounted for only 4.8$\%$ of all data points. Figure~\ref{fig:hypo1} shows the outcome of linear regression between the empirical probabilities and displayed ratings. The coefficient of determination $R^2=0.9522$ suggests a strong correlation. The positive slope suggests a positive correlation, and the negative intercept suggests that participants would not follow the recommendations when the displayed rating is less than $\frac{0.2113}{0.2397} \approx 0.9$. In the extreme case when the quantized display rating is $5$, the linear regression model generates a projected empirical probability of $0.9872$ which is consistent with the theoretical model in \eqref{eq:p flow dynamics-m-general-matrix}.

\subsection[]{Long Run Behavior of \(\hat{P}\)}
\label{sec:Phat}
Recall that $\hat{P}^s$ is held constant throughput the session of participant $s$, and updated to $\hat{P}^{s+1}$ at the end of the session. Also, note from the definition that $\hat{P}^s$ is a row-stochastic matrix, and that its diagonal entries are zero. In our current case of $\nlinks=3$, this therefore leaves $3$ independent entries, say $\hat{P}^{s}_{12}, \hat{P}^{s}_{23}$ and $\hat{P}^{s}_{31}$. The evolution of these quantities with increasing $s$ is shown in Figure~\ref{fig:hypo1_P}. The plots suggest convergence of $\hat{P}^s$ as $s$ increases.

\begin{figure}[htb!]
\begin{center}
\begin{minipage}[c]{.3\textwidth}
\begin{center}
\includegraphics[width=1.0\textwidth]{P12} 
\end{center}
\end{minipage}
\begin{minipage}[c]{.3\textwidth}
\begin{center}
\includegraphics[width=1.0\textwidth]{P23} 
\end{center}
\end{minipage}
\begin{minipage}[c]{.3\textwidth}
\begin{center}
\includegraphics[width=1.0\textwidth]{P31} 
\end{center}
\end{minipage}
\end{center}
\caption{\sf Evolution of $\hat{P}^s$ with participant number $s$.}
\label{fig:hypo1_P}
\end{figure}

%All 3 independent entries, thus $P^{\#n}$, clearly tend to converge, though with some oscillations which might be resulted from the small number of total participants. 

%\begin{result}
%There exists a strong positive correlation between the compliance rate and quantized average review rating. There is evidence of convergence of $P^{\#n}$.
%\end{result}

\subsection{Long Run Behavior of the Displayed Rating}
\label{sec:displayed-rating}
\begin{figure}[htb!]
\begin{center}
\begin{minipage}[c]{.475\textwidth}
\begin{center}
\includegraphics[width=1.0\textwidth]{hypo2_rating} 
\end{center}
\end{minipage}
\end{center}
\caption{\sf Evolution of end of session display rating $r^s(100)$ with participant number $s$.}
\label{fig:hypo2_rating}
\end{figure}

Recall from \eqref{eq:human-output-to-input-1} that in order to simulate review collection from multiple participants participating simultaneously, we rather collect reviews from previous scenarios by previous participants who made route choice under the same realization of state and for the same displayed rating. Naturally, the accuracy of such a surrogate becomes better with more data collection. Motivated by this, we studied the long run behavior of displayed rating $r^s$ in two ways. First, we studied the end of session displayed rating with increasing participant number. As Figure~\ref{fig:hypo2_rating} illustrates, that this value increases to roughly $4.67$, and seems to be settling around this value, by the last participant. 
%Since the participants participated sequentially, we simulated the simultaneous routing behavior of multiple participants by incorporating submitted review ratings of all past participants, under the same realized state of nature and the same quantized average review rating (quantization step = 0.5), when updating the average review rating after the current participant submitted his or her review rating. That means as the number of participants grows, more and more historical data will be used to update the average review rating. Roughly speaking, the evolution of average review rating of the $n$-th participant's session includes information of that of all previous $n-1$ participants.
%
%We set initial average review rating equal to 2.5 (out of 5) for all participants. First, we studied the average review rating at fixed 100-th scenario (at the end of each experiment session) for different participants. Figure~\ref{fig:hypo2_rating} shows the asymptotic behavior of average review rating  as the number of sessions (participants) grows.
%The average review rating of the 100-th scenario for participants $\#1$ was around 4.34. As the number of sessions (participants) grows, the endgame average review rating grows, with minor oscillations, and converges around 4.67. Since we only collected useable data of 33 sessions (participants), we expect the endgame average review rating to further grow as more and more sessions are conducted. However, getting the endgame average review rating finally converge to 5, which means almost all submitted review ratings equal to 5, is somehow unrealistic.
Second, we studied the displayed rating during the session of the last participant participant $\#33$. Figure~\ref{fig:hypo2_rating_34} shows a monotonic increase of the displayed rating from $2.5$ (recall that the initial condition is set to be $r^s(1)=2.5$ for all the participants) to a value of around $4.67$ by the end of the session. The evolution of display rating is understandably smoother given that the set $\bar{\mc R}$ used in \eqref{eq:human-output-to-input-1} has sufficient samples for all frequently occurring combinations of $\omega$ and $r$ by the time of the last participant. 

%provides a more intuitive perspective of the asymptotic behavior of average review rating as the number of scenarios grows.
%The average review rating of the first scenario for participant $\#34$ is 2.5. As the number of scenarios grows, the average review rating grows and converges around 4.67 at the 100-th scenario.

\begin{figure}[htb!]
\begin{center}
\begin{minipage}[c]{.475\textwidth}
\begin{center}
\includegraphics[width=1.0\textwidth]{hypo2_rating_34} 
\end{center}
\end{minipage}
\end{center}
\caption{\sf Evolution of the display rating during the session of the last participant, i.e., $r^{33}(k)$, with scenario number $k$.}
\label{fig:hypo2_rating_34}
\end{figure}

\subsection{Long Run Empirical Probability of Following Recommendation}
\label{sec:following}
Figure~\ref{fig:hypo2_rate} shows the evolution of cumulative empirical probability of following recommendations from the start of session for participant 1 through the end of session for $s$ for increasing value of $s$. 

%We also studied the asymptotic behavior of cumulative compliance rate at the end of each experiment session (the 100-th scenario) as the number of sessions (participants) grows as in Figure~\ref{fig:hypo2_rate}.
\begin{figure}[htb!]
\begin{center}
\begin{minipage}[c]{.475\textwidth}
\begin{center}
\includegraphics[width=1.0\textwidth]{hypo2_rate} 
\end{center}
\end{minipage}
\end{center}
\caption{\sf Evolution of end of session cumulative empirical probability of following recommendation with increasing participant number.}
\label{fig:hypo2_rate}
\end{figure}

This cumulative empirical probability in Figure~\ref{fig:hypo2_rate} seems to converge to around $0.87$. This compares very well with the prediction of the linear regression model of Section~\ref{sec:hypo1}, according to which the empirical probability of following recommendation for the display rating of $4.67$ (the long run value from Section~\ref{sec:displayed-rating}) is approximately equal to $0.2397\times 4.67-0.211=0.91$. 
%As the number of sessions (participants) grows, the cumulative compliance rate grows and converges to around 0.87.  Using the linear regression model in Section~\ref{sec:hypo1} and the steady-state endgame average review rating of 4.67, we can compute the theoretical steady-state compliance rate $\approx 0.91=0.2397\times 4.67-0.211$. The theoretical and actual steady-state compliance rate are close to each other, which again verifies the validity of the linear regression model in Section~\ref{sec:hypo1}.

%\begin{result}
%The endgame average review rating converges to 4.67 while the cumulative compliance rate converges to 0.87, based on data of 33 sessions, each consists of 100 scenarios.
%\end{result}

\subsection{Displayed Rating vs Time-Averaged Aggregated Regret}
\label{sec:display-vs-aggregated-regret}
%To study the relation between submitted review rating and regret, we have to define regret properly. In our previous theoretical work, the regret model requires knowledge of $P$, which can only be computed using historical data of all previous participants and is inaccessible to the current participants. Based on the available information in our user interface, which consists of actual travel times of all 3 routes, we redefined the individual regret as the difference between the actual travel time of recommended route and fastest route.

%When updating the average review rating, submitted review ratings of all past participants, under the same realized state of nature and the same quantized average review rating (quantization step = 0.5) as the current participants' current scenario are averaged to get the new average review rating. In order to properly grasp the relation between the average review rating and regret, the regret should be averaged over all individual regrets of all past participants, under the same realized state of nature and the same quantized average review rating accordingly.

%The new definition of time-averaged aggregated regret makes it a non-negative value. As time-averaged aggregated regret becomes larger, we expect average review rating to be lower, or the deducted average review rating to be larger. 
Based on the data from all the 3300 scenarios, we could not find a good  correlation between the displayed rating and time-averaged aggregated regret (no regression model gave a good fit). We then repeated analysis after discarding the data which satisfy at least one of the following (for reasons similar to the one described in Section~\ref{sec:hypo1}): 
\begin{itemize}
\item The displayed rating was less than $4$. This was to remove the transient effect from initial condition $r^s[1]=2.5$. This accounted for only about 5 \% of total data points. 
\item The time-averaged aggregated regret (cf. \eqref{eq:subject-model}) is less than $2.6$ minutes. This was because the displayed ratings varied vastly during such scenarios. This accounted for about 50 \% of total data points. 
\end{itemize}

%We first discarded all 164 ($\approx 5.02\%$) data points whose average review rating $R^{\#n}[k+1]<4$ in order to eliminate the impact of initialization. Those data are generated in the beginning of experiment sessions, and are heavily influenced by the initial value we set $R^{\#n}[1]=2.5$. 
%We observe that, when time-averaged aggregated regret is less than certain value $x$, that is when the recommended route is less than $x$ minutes slower than the fastest route, average review ratings vary vastly and show no clear correlation with the time-averaged aggregated regret. After discarding data that has regret less than 2.6547 (1661 data $\approx$ 50.84\% data), 
%
Figure~\ref{fig:hypo3} (e) shows the outcome of linear regression between the displayed rating and the corresponding time-averaged aggregated regret values after pre-processing the data using aforementioned threshold values. The $R^2=0.6167$ value suggests a moderate negative correlation. Figure~\ref{fig:hypo3} also shows linear regression outcomes using different combinations of threshold values. For example, Figure~\ref{fig:hypo3} (f) shows the regression after discarding data with displayed rating less than 4, or when the time-averaged aggregate regret is less than 4 minutes, and that this resulted in retaining 1\% of total data points. The scenario in Figure~\ref{fig:hypo3} (e) gives the maximum $R^2$ value. 

\begin{figure}[htb!]
\begin{center}
\begin{minipage}[c]{.3\textwidth}
\begin{center}
\includegraphics[width=1.0\textwidth]{hypo3_1} 
(a) \, (0, 2.25, 100\%)
\end{center}
\end{minipage}
\begin{minipage}[c]{.3\textwidth}
\begin{center}
\includegraphics[width=1.0\textwidth]{hypo3_2} 
(b) \, (2.6, 2.25, 46\%)
\end{center}
\end{minipage}
\begin{minipage}[c]{.3\textwidth}
\begin{center}
\includegraphics[width=1.0\textwidth]{hypo3_3} 
(c) \, (4, 2.25, 1\%)
\end{center}
\end{minipage}
\end{center}
\begin{center}
\begin{minipage}[c]{.3\textwidth}
\begin{center}
\includegraphics[width=1.0\textwidth]{hypo3_4}
(d) \, (0, 4, 95\%) 
\end{center}
\end{minipage}
\begin{minipage}[c]{.3\textwidth}
\begin{center}
\includegraphics[width=1.0\textwidth]{hypo3_5} 
(e) \, (2.6, 4, 44\%)
\end{center}
\end{minipage}
\begin{minipage}[c]{.3\textwidth}
\begin{center}
\includegraphics[width=1.0\textwidth]{hypo3_6} 
(f) \, (4, 4, 1\%)
\end{center}
\end{minipage}
\end{center}
\begin{center}
\begin{minipage}[c]{.3\textwidth}
\begin{center}
\includegraphics[width=1.0\textwidth]{hypo3_7} 
(g) \, (0, 4.6, 33\%)
\end{center}
\end{minipage}
\begin{minipage}[c]{.3\textwidth}
\begin{center}
\includegraphics[width=1.0\textwidth]{hypo3_8} 
(h) \, (2.6, 4.6, 13\%)
\end{center}
\end{minipage}
\begin{minipage}[c]{.3\textwidth}
\begin{center}
\includegraphics[width=1.0\textwidth]{hypo3_9} 
(i) \, (4, 4.6, 0\%)
\end{center}
\end{minipage}
\end{center}
\caption{\sf Relation between displayed rating and time-averaged aggregated regret for all participants.}
\label{fig:hypo3}
\end{figure}

We also investigated correlation on an individual participant basis. We found that a large number of participants submitted $\Rmax=5$ review too often. Indeed, only 9 out of the 33 participants submitted review of $5$ less than half of their individual 100 scenarios. This might be because the default review on the slider is set to $5$ before the participant adjusts it to submit his/her own review, and hence data from participants who submit a review $5$ too often might be biased. 

%Since we set the default value of review rating equal to 5, submitting 5 (full) review rating too often may suggest that the participant is choosing his or her review rating carelessly. So we studied the relation between average review rating and regret on participant base, only using data from those 9 careful participants.

%we discarded data associated with irrationality. The first category of irrational data are those when participants deducted rating (submitted rating $<$ 5) even though the regret is 0 (the recommended route is the fastest route). The second category of irrational data are those when participants submitted 5 (full) review rating even though the regret is nonzero (the recommended route is not the fastest route). After eliminating irrational data (usually consists of more than half of the data), 

Analysis of data on an individual basis from $9$ participants who submitted review of $5$ less than half times revealed that, for $5$ of such participants, there was a strong negative correlation ($R^2>0.93$) between displayed rating and time-averaged aggregated regret. This relationship for one such participant ($\#21$) is shown in Figure~\ref{fig:hypo3_22}, where we discarded data points ($\approx 4\%$ of total data) when the review rating was less than $4$ to remove the transient effect from initial condition $r^{21}(1)=2.5$. The average $R^2$ value\footnote{The \emph{average $R^2$ value} for multiple participants refers to the average of the $R^2$ values computed for individual participants.} for all the $9$ participants who submitted review of $5$ less than half times was $0.649$. On the other hand, the average $R^2$ value for the other $24$ participants who submitted review of $5$ more than half times was $0.4664$.
%When we study the individual correlation between the deducted average review rating and time-averaged aggregated regret, 5 out of those 9 careful participants has a coefficient of confidence $R^2>0.93$. For example, the relation between the deducted average review rating and time-averaged aggregated regret for participant $\#22$ is shown in Figure~\ref{fig:hypo3_22}.

\begin{figure}[htb!]
\begin{center}
\begin{minipage}[c]{.475\textwidth}
\begin{center}
\includegraphics[width=1.0\textwidth]{hypo3_new_22} 
\end{center}
\end{minipage}
\end{center}
\caption{\sf Relation between displayed rating and time-averaged aggregated regret for a sample participant.}
\label{fig:hypo3_22}
\end{figure}

We repeated our analysis by taking into account participants' response to feedback survey, specifically to questions 6 and 7 (see Appendix). $12$ participants self-reported to be using the  strategy suggested in pre-experiment instructions for making route choice decision by carefully taking into account recommended route, displayed rating and histograms. The remaining $21$ participants self-reported to be following recommendations if the displayed rating is above a threshold value. The average of this self-reported threshold value was $4.175$.

We analyzed the data separately for these two types of participants. After discarding data points corresponding to displayed rating less than $4$, analysis of the remaining data from the $12$ participants who used the strategy suggested in the instructions revealed a moderate negative correlation between displayed rating and time-averaged aggregated regret (average $R^2$ = $0.5897$). For $5$ of such participants, there was a strong negative correlation (average $R^2>0.93$). On the other hand, for the rest $21$ participants who used threshold based strategy, their average $R^2$ value was $0.4708$. 

There were $2$ participants who self-reported to use the recommended strategy, and also submitted review of $5$ less than half times. The average $R^2$ value for these $2$ participants was $0.9505$, suggesting a strong (negative) correlation between displayed rating and time-averaged aggregated regret for them.

%After discarding initialization data that has average review rating less than 4 (4 data $\approx$ 4.04\% data), the relation between average review rating and regret for participant $\#22$ is highly linear.


%Notice that, those two categories of irrational data, even among the 9 careful participants, usually appears in more than half of the scenarios. For example, for participant \#6 in Figure~\ref{fig:hypo3}, 65 out of 100 scenarios can be categorized into either of those two irrationality categories, while only 35 out of 100 scenarios generates careful and rational data. Even when we analyzed rational data for a specific careful participant, the largest coefficient of confidence we can get is poorly 0.5289. What is even worse is that the quadratic regression model is non-monotonic which contradicts with the presumably monotonic increasing relation between the deducted rating and regret. Even though we can try to redefine the notion of regret once again to try to get a better fit, but perhaps after all, participants' submitted review ratings are strongly subjective and irrational.

%\begin{result}
%%There exists a moderate positive correlation between the average review rating and time-averaged aggregated regret. 
%The correlation is particularly strong for those careful participants who submitted 5 (full) review ratings less than half of the time.
%\end{result}

==> An Experimental Study on Learning Correlated Equilibrium in Routing Games/hypotheses-ks.tex <==
\section{Adapting Theory to Experiment Setup and Hypotheses}
\label{sec:adapting}
Let there be $\numsubjects$ human participants in total, each participating for $\numscenarios$ rounds. The numbering of the participants is in the order in which they participate. Figure~\ref{fig:blockdiagram} shows that the response from a participant in every round consists of route chosen in that round as well as the review about the quality of recommendation in that round. In Section~\ref{sec:theory}, we provided a model for an estimate of this review to be related to a notion of instantaneous regret. We modify the notion for the experiments as follows. Let $\ell_1, \ldots, \ell_{\nlinks}$ be the realized travel times on the $\nlinks$ links, and let $j$ be the recommended route. Then, we let instantaneous regret be equal to $\ell_j - \min_{i \in [\nlinks]} \ell_i$. 

\begin{figure}[htb!]
\begin{center}
\include{fig/block-diagram}
\caption{\sf Input-output illustration for the participant and the simulated model.}
\label{fig:blockdiagram}
\end{center}
\end{figure}


The responses of the participants are summarily stored and updated as follows:
\begin{itemize}
\item $\mc R(s,k;\omega,r)$: set of the reviews submitted by participants $1, \ldots, s-1$ in all their rounds $1, \ldots, \numscenarios$, and by participant $s$ in rounds $1, \ldots, k$,  when the state realization was $\omega$, and the displayed rating was $r$. Let $\bar{\mc R}(s,k;\omega,r)$ be the average of those review values.
\item $\mc M(s,k;\omega,r)$: set of instantaneous regret for participants $1, \ldots, s-1$ in all their rounds $1, \ldots, \numscenarios$, and by participant $s$ in rounds $1, \ldots, k$, when the state realization was $\omega$, and the displayed rating was $r$. Let $\bar{\mc M}(s,k;\omega,r)$ be the average of these regret values.
\item $\mc N(s;i,j)$: number of times participants $1, \ldots, s-1$ choose route $j$ when recommended route $i$ in all their rounds $1, \ldots, \numscenarios$.
\end{itemize}

Furthermore, the matrix $P$ is intrinsic to the participants and needs to be estimated online during the experiments. We adopt the following natural estimate: 
%\begin{equation*}
%\hat{P}_{ij}^{s}= \frac{\mc N(s;i,j)}{\sum_{j \in [\nlinks]} \mc N(s;i,j)}, \quad i, j \in [\nlinks], \quad s \in \{2, \ldots, \numsubjects\}
%\end{equation*}
\begin{equation*}
\hat{P}_{ij}^{s}= \begin{cases}\frac{\mc N(s;i,j)}{\sum_{j \in [\nlinks], j\neq i} \mc N(s;i,j)} & i\neq j \\ 0 & i=j \end{cases} \quad i, j \in [\nlinks], \quad s \in \{2, \ldots, \numsubjects\}
\end{equation*}
starting with a specified $\hat{P}^1$ for the first participant. 

The ratings to be displayed as well as link flows for the human participant $s \in [\numsubjects]$ in various rounds are given by\footnote{The rating $r^s$ is quantized to the nearest first decimal place when displaying to the participants.}: for $k = 1, \ldots, \numscenarios-1$, 
\begin{align}
r^s(k+1) & =  \frac{k}{k+1} r^s(k) + \frac{1}{k+1} \, \bar{\mc R}(s,k;\omega(k),r^s(k)) \label{eq:human-output-to-input-1} \\
f^s_i(k+1) & = \pi_{\omega(k+1),i} \frac{r^{s}(k+1)}{\Rmax} + \sum_{j \in [\nlinks]} \hat{P}^{s}_{ji} \pi_{\omega(k+1),j} \left(1-\frac{r^{s}(k+1)}{\Rmax}\right) \label{eq:human-output-to-input-2}
\end{align}
starting with a specified $r^s(1)$ for the first round. 

We modify the model for human participant from \eqref{eq:instant}-\eqref{eq:S-agent-update} as: $k = 1, \ldots, \numscenarios$,
\begin{equation}
\label{eq:subject-model}
\begin{split}
\hat{u}^s(k) & = \bar{\mc M}(s,k;\omega(k),r^s(k)) \\
\hat{m}^s(k) & = \frac{1}{k} \left(\hat{u}^s(1) + \ldots + \hat{u}^s(k) \right)
\end{split}
\end{equation}

\subsection{Hypotheses}
%\ksmarginphantom{need to pick one from obey/comply/follow} \yzmarginphantom{used follow after section II, did not touch abstract/introduction}
Our objective is to test the following hypotheses:
\begin{enumerate}
\item[(H1)] Empirical probability of a participant choosing recommended route is proportional to the value of the rating displayed with the recommendation. The findings for this hypothesis are in Section~\ref{sec:hypo1}.
\item[(H2)] The displayed rating, i.e., $r^{s}(\cdot)$, converges to its maximum value $\Rmax$ as $s$ increases. The empirical probability of participants choosing recommended route converges to $1$ as $s$ increases. The findings for this hypothesis are in Sections~\ref{sec:displayed-rating} and \ref{sec:following}.
\item[(H3)] The empirical distributions of route choices when not following recommendation, i.e., off-diagonal entries of $\hat{P}^s$, converge as $s$ increases. The findings for this hypothesis are in Section~\ref{sec:Phat}.
\item[(H4)] There is a negative correlation between time-averaged aggregated regret $\hat{m}^{s}(\cdot)$ and the displayed rating $r^s(\cdot)$. The findings for this hypothesis are in Section~\ref{sec:display-vs-aggregated-regret}.
\end{enumerate}

%\subsection{A Pseudo-Non-atomic Setup for Experiments}
% Accordingly, the following modifications are made:
%\begin{itemize}
%\item $P$ serves two purposes: estimating the regret of an agent in \eqref{}, and thereby the cumulative regret in \eqref{}, and hence the obedience rate as per our hypothesis, and, for a given obedience rate, to forecast the cumulative flow induced in the links by all the agents. 
%\end{itemize}
%

%Let $\state \sim \prior \in \interior(\triangle(\allstates))$, for some prior $\prior$ which can be inferred from the histogram information that is accessible to all the participants. The participants do not have access to the realization of $\state$, but all participants receive private route recommendations conditional on the realized state. These conditional recommendations are generated by a \emph{diagonal atomic}~\cite{Zhu.Savla:TCNS22} \emph{signal} $\signal=\{\signal^{\state} \in \simplex_3: \, \state \in \allstates\}$. 
%In the experiment study, we specifically choose the following parameters: $\mu_0(\omega_1)=0.1, \mu_0(\omega_2)=0.2, \mu_0(\omega_3)=0.4, \mu_0(\omega_4)=0.05, \mu_0(\omega_5)=0.25$, \begin{equation*}
%\pi = 
%\kbordermatrix{&i=1&i=2&i=3\\
%\omega_1&0.1&0&0.9\\
%\omega_2&0&1&0\\
%\omega_3&0.6&0&0.4\\
%\omega_4&0.9&0.1&0\\
%\omega_5&0.6&0.4&0\\}
%\end{equation*}



%\subsection{Hypotheses}
%We want to show that, if the route recommendation strategy adopted by the platform satisfies a certain obedience property, then under the above model, the participants compliance rate will become 100\% in the long run. A strategy is said to satisfy the obedience property if every route recommendation generated by this strategy is best on average a posteriori for the participant who receives it. Note the emphasis on average in the definition of obedience property, whereas we aim for full compliance in the long run in every scenario.
%
%Our hypotheses are listed below.
%
%\begin{hypothesis}
%Participants follow recommendations with a probability proportional to the average star rating $R^{\#n}(k)$. When they do not follow the recommendation, their route choice profile $P^{\#n}_{ij}$ converges to a constant conditional probability distribution.
%\end{hypothesis}
%
%\begin{hypothesis}
%The displayed average star rating $R^{\#n}[t]$ becomes 5 stars, and the compliance rate becomes 100\% in the long run.
%\end{hypothesis}
%
%\begin{hypothesis}
%There exist some relationship between average review rating $R^{\#n}(k+1)$ and time-averaged aggregated regret $\tilde{m}^{\#n}(k)$.
%\end{hypothesis}

==> An Experimental Study on Learning Correlated Equilibrium in Routing Games/implementation-ks.tex <==
\section{Experiment Procedure}
\label{sec:procedure}
%\ksmargin{need to change from subject/agent/user to participant} 
%\yzmargin{used agent in section II, used participant after section III, did not touch abstract/introduction}
Simulating non-atomic setup requires simultaneous participation by a very large number of participants. Practical limitations on laboratory experiments therefore necessitate consideration of a pseudo-non-atomic setup, consisting of mixture of a small number of human participants and a large number of simulated participants. We performed experiments in the limiting case of one human participant at a time with change of participant after a fixed number of rounds.

The experiment protocol was reviewed and approved by the Institutional Review Board at the University of Southern California (USC \# UP-22-00107). 
The experiment was conducted in the Kaprielian Hall at USC during April 2022 and May 2022. A total of 34 participants with a good command of the English language and with no prior experience with our experiment were recruited from the undergraduate population of the university. Upon arrival at the laboratory, participants were given a presentation by an experiment personnel, aided by slide illustrations, available at \cite{RoutingExpSlides}. 
The experiments was run on a networked desktop computer, and programmed using Python. \yzmarginphantom{Asked Christine for detailed info regarding the programming software and database, waiting for the reply.} Except for experiment personnel, only one participant was present in the laboratory during an experiment session. 

\begin{figure}[htb!]
\begin{center}
\begin{minipage}[c]{.475\textwidth}
\begin{center}
\includegraphics[width=1.0\textwidth]{interface1} 
\end{center}
\end{minipage}
\end{center}
\caption{\sf User interface before route selection during a typical scenario.}
\label{fig:user-interface-1}
\end{figure}

During the experiment, a participant had to select one among three routes in a traffic network on computer, in a series of rounds or \emph{scenarios}. The traffic network was chosen to be outside the Los Angeles area to minimize bias. 
The information displayed during a typical scenario, as shown in Figure~\ref{fig:user-interface-1}, consisted of: (i) Traffic network with three possible routes to go from the origin to the destination, marked as Route 1, Route 2, and Route 3. The route highlighted is the recommended route; (ii) Travel time forecasts on different routes corresponding to different underlying states, shown via histogram in the right side of the screen; (iii) Average rating at the top left indicating what other participants in the past thought of the quality of recommendation in terms of recommending the fastest path. The average rating is on a scale of 1 to 5 with 5 being the highest; and (iv) Menu at the bottom to enter route selection. During the pre-experiment presentation, the participants were instructed to make route choice based on the information contained in (i)-(iii). Specifically, they were instructed to let their likelihood of following the recommendation be proportional to the displayed rating, and to use the histogram when they decide not to follow the recommendation. Upon selecting a route, and pressing the "Select" button, the computer revealed the \emph{actual} travel time on top of the histogram for each route as in Figure~\ref{fig:user-interface-2}. These are the forecasts for the specific state value associated with the round. 

%\yzcomment{During the pre-experiment presentation, the participants were instructed to make route choice based on the information contained in}
%Specifically, they were instructed to follow the recommendation with a probability proportional to the displayed rating, and use the histogram when they decide not to follow the recommendation.}

\ksmarginphantom{check Figures~\ref{fig:user-interface-1} and \ref{fig:user-interface-2} for why the histograms are incomplete}
\begin{figure}[htb!]
\begin{center}
\begin{minipage}[c]{.475\textwidth}
\begin{center}
\includegraphics[width=1.0\textwidth]{interface2} 
\end{center}
\end{minipage}
\end{center}
\caption{\sf User interface after route selection and before review submission during a typical scenario.}
\label{fig:user-interface-2}
\end{figure}

The travel time forecasts are computed from \emph{forecasted} link flows using the link latency functions in \eqref{eq:polynomial-latency-function}, where the state $\omega$ is predetermined and is the same for all the participants in the same round. The forecasted link flows are computed by assuming that the other agents follow recommendation with a likelihood proportional to the displayed rating, and for those who do not follow, their route choice mimics the alternate choices made by previous participants under same state and same displayed rating; see \eqref{eq:human-output-to-input-1}-\eqref{eq:human-output-to-input-2} for details.
%The sampled sequence satisfies that the empirical probability distribution is the same as the prior $\mu_0$. 
 The participant is required to enter his/her own experience with the quality of recommendation in this scenario by choosing a review rating on a sliding scale at the bottom of the screen. During the pre-experiment presentation, the participants were instructed to consider not only the rankings but also the difference in values of actual travel times of both the recommended route and the route chosen by participants to come up with a rational review rating.
Upon pressing the "Rate" button, the computer showed the next scenario whose displayed rating is the average of the review just submitted by the participant and the reviews submitted by previous participants under same state and same displayed rating; see \eqref{eq:human-output-to-input-1} for details. The process repeats until all the scenarios are done, after which the participant was asked to fill a survey to get insight into his/her route choice decision making strategy during the experiment. This survey is provided in the Appendix.

\ksmarginphantom{need to provide some justification for this choice of performance}
All participants received a show-up renumeration of US \$10 and an additional maximum of US \$10 depending on the \emph{level of homogeneity} that they exhibit. For a given participant, this is measured in terms of the difference between his/her empirical conditional route choice probability distributions and that of the previous participants. This is then mapped proportionally to the renumeration amount. The conditional probability distribution here refers to the probability of choosing route $j$ when recommended route $i$. The additional renumeration averaged \$9.5 across all participants. We used a pretty generation mapping from a participant's level of homogeneity to his/her renumeration, and therefore the high average is not necessarily an indication of high level of homogeneity among the participants.  All the renumeration was paid in cash. 
%The average total renumeration per participant came out to be US \$19.5. \yzcomment{Note that, this high average renumeration value is not a direct indicator of a high level of average performance, because it is a result of both the choice of renumeration constant and the actual average level of performance.} 
Participant sessions lasted for approximately an hour on average. 

For each scenario, we recorded the displayed rating (between 0 and 5), the recommended route ($\{1,2,3\}$), the selected route ($\{1,2,3\}$), the submitted review (between 0 and 5), the start and end times (the local clock time of the computer running the experiment program).

==> An Experimental Study on Learning Correlated Equilibrium in Routing Games/introduction-ks.tex <==
\section{Introduction}
Route choice decision making in traffic networks with travel time uncertainties is a challenging task for drivers. The uncertainties, e.g., due to traffic incidents, are hard to predict and even if known are hard to incorporate optimally into real-time decision-making by the drivers. Therefore, route recommendation platforms are compelling options in such settings. The information advantage of such platforms, i.e., almost real time information about the incidents, combined with availability of huge computational resources, and the ability to make private recommendations, e.g., through mobile devices, also gives these platforms the possibility to steer the driver decisions towards a desired objective. The efficacy however depends on the extent to which the drivers follow the recommendations. This aspect is ignored in typical route recommender systems, e.g., see \cite{Wang.Li.ea:14,Herzog.Massoud.ea:17}.
\emph{Information design}, e.g., see \cite{Bergemann.Morris:19}, provides a framework to formalize the act of following recommendation through the notion of \emph{obedience}. A \emph{private signal}, i.e., mapping from the state to distribution over private recommendations is called obedient in a one-shot game, if following the recommendation leads to smallest travel time in expectation a posterior. The corresponding outcome in the form of link flows is the correlated equilibrium induced by the signal.  

A plausible extension of obedience to repeated setting is that the likelihood of following recommendation in a round is related to \emph{regret} from previous rounds. If the regret is of satisficing type with respect to a default choice and is averaged over past rounds and over all agents, then the asymptotic outcome under an obedient recommendation policy is known to coincide with the one-shot outcome~\cite{Zhu.Savla:DGAA21}. Moreover, this \emph{learning rule} does not require explicit knowledge of the signaling policy by the agents. However, there has been no experimental study of such learning rules or even of correlated equilibrium for non-atomic games to the best of our knowledge. 

There has been a lot of theoretical work on learning Nash equilibria in the context of selfish routing, e.g., see \cite{Fischer.Racke.ea:10,Blum.Even-Dar.ea:10,Krichene.Drighes.ea:15}. There has also been experimental investigation on convergence of route choice behavior to Nash equilibrium, e.g., see \cite{Iida.Akiyama.ea:92,Selten.Chmura.ea:07}. However, corresponding work on correlated equilibria are lacking. In face, existing experimental studies on correlated equilibrium are almost exclusively for 2 X 2 settings and concern primarily Game of Chicken and the Battle of Sexes, e.g., see \cite{Cason.Sharma:07,Duffy2010,Bone.Drouvelis.ea:12,Duffy2017,Arifovic.Boitnott.ea:19}. These studies have identified the following to be key drivers for ensuring high rate of following recommendation: (i) clear and common understanding of the signal which generates the recommendations, often achieved by public announcement of the signaling policy; (ii) the induced correlated equilibrium being Pareto improvement over Nash equilibria; (iii) accurate knowledge of mapping between utility and payoffs of players; (iv) trust that the opponent will follow the recommendation; and (v) fixed vs. random opponent in different rounds, with the former allowing development of strategy profile of the opponent and using it for choice of action. Other studies include \cite{Anbarci2018} which examined the effect of payoff asymmetry on a participant's willingness to follow recommendations.
%, \kscomment{and \cite{Oprea2011} which found participant's play converges to mixed or pure Nash equilibrium under different conditions which supports predictions of evolutionary game.} \ksmargin{is \cite{Oprea2011} relevant?}

Some of the considerations mentioned above in the context of following recommendations become more significant for non-atomic games. 
Signaling policies for these games comprise probability distributions with continuous support. This complexity makes the announcement of signal by the mediator as well as its comprehension by the participants to be challenging. This may potentially aggravate known issue with participants not able to execute Bayes rule accurately even for probability mass functions. The issue of trust that other participants will follow recommendations takes assumes a bigger role in the presence of continuum of participants. Furthermore, practical limitations on laboratory experiments necessitates consideration of a pseudo-non-atomic setup, consisting of mixture of a small number of human subjects and a large number of simulated agents. We performed experiments in the limiting case of one human subject at a time with change of participant after a fixed number of rounds.

%Previous theoretical and empirical studies (not restricted to traffic networks) have shown that, in the presence of a coordinator, the action profiles of a few (typically two) competing agents converges to a correlated equilibrium. This is an action profile at which, under the public knowledge of the coordination strategy, no individual agent has an incentive to deviate unilaterally. The agent decision making model in such studies is typically of the kind where, in each round, the agent selects an action which is best response to the opponent?s actions in the past. In traffic network, where the agents/drivers are numerous, it is unrealistic for an individual driver to keep track of past route choice decisions of all the other drivers. It is perhaps more realistic to keep track of travel times of different routes which results from the collective decisions of all the drivers. Moreover, the presence of publicly available review rating gives an additional information about the compliance rate of the driver population towards accepting the route recommendations of the coordinator, i.e., the recommendation platform, in the near future. In recent theoretical studies, we have shown that even in this setting, for a properly chosen coordination strategy, the route choice of the drivers converges to being consistent with correlated equilibrium associated with the coordination strategy, or equivalently the compliance rate becomes 100\% in the long run. 

The outline of our experiments is as follows. One participant at a time engages in repeated route choice decision on computer. In every round, one of five states is i.i.d. sampled according to a probability distribution. The participant is shown travel time forecasts for each of the three routes for the five possible underlying states, a route recommendation generated by an obedient policy conditional on the state realized, and a numeric rating suggestive of average experience of previous participants with the quality of recommendation they received during rounds with the same realized state. The travel time forecasts are based on the assumption that the fraction of other agents who follow recommendation is proportional to the displayed rating, and those who do not follow mimic empirical route choice collected from previous participants. Once the participant enters route choice, the actual travel times on the routes are revealed. These are the  forecasted travel times for the specific state value associated with the round. 
The participant uses this information to evaluate the quality of recommendation received in the round and enters a numeric review accordingly. This is combined with historical reviews to update rating for the next round. 
%
%In this study, we propose to test this hypothesis in a simulated environment. Instead of subjects participating simultaneously, we shall have them participate sequentially. Each participant will make route choice decisions in a sequence of scenarios which differ in terms of type of incident, and hence also route recommendation. The information displayed to the n-th participant (travel time, review rating) for a particular scenario will include the effect of route choice decisions of previous n-1 participants under the same scenario. At the end of each scenario, the participant makes a route choice decision. Thereafter, the simulation reveals the actual travel times on all paths by taking into consideration decisions by previous n-1 participants in similar scenarios. The participant then provides a rating on his/her perception of the quality of recommendation received in the previous round. The simulation then switches to the next round and the process repeats until the end of the experiment. 
At the conclusion of all its rounds, the participant is asked to fill out a feedback survey, which is designed to get insight into the participant's decision making strategy. Our strategy to announce payoffs, i.e., travel times, is equivalent to announcing the signal. Announcing \emph{forecasted} payoffs based on actual decisions by previous participants, instead of \emph{equilibrium} payoffs in conjunction with rating is meant to elicit trust, and hence recommendation following from the participants. 
%\kscomment{The display rating and its update provides an another indicator of what other participants thought in the past.} 
Data from 33 participants each with 100 rounds was analyzed to investigate the correlation between empirical probability of following recommendation by the participants, regret, as well as the displayed rating, and the convergence of displayed rating and the empirical distribution of route choice by the participants. 

%Our experimental study uses ~\cite{Anbarci2018}, ~\cite{Duffy2017}, ~\cite{Oprea2011} and ~\cite{Duffy2010} for reference in the process of designing our recruitment requirements and scale, the experiment length and compensation method and amount.

Our main contributions and findings are as follows. First, we provide an experiment protocol template for studying correlated equilibrium in non-atomic games. Second, through our experimental findings, we provide an instantiation of a setting in which the long run route choice decisions are highly consistent with private recommendations generated by an obedient policy. 
Our third contribution is in verifying elements of a prior dynamic model for obedience in multi-round setting. Our experiments found strong correlation between following recommendation in a particular round and the display rating in that round. We found moderate correlation overall between the review submitted by a participant in a round and the regret which could be associated with the outcome of the round. This correlation however became strong when restricted to participants who demonstrated and self-reported to carefully assess all the information for their route choice decision and for providing review feedback. 
This is important because the notion of regret has been a mainstay in prior theoretical studies on convergence to correlated equilibrium. Overall, the displayed rating converged to maximum value in conjunction with very high likelihood of following recommendation. 

The rest of the paper is organized as follows. Section~\ref{sec:theory} gives the necessary background on modeling and analysis of non-atomic routing game which forms the basis for experiment design. Section~\ref{sec:procedure} provides a general overview of the experiment protocol, while connection with the non-atomic setup and hypotheses are presented in Section~\ref{sec:adapting}. Experimental findings are presented in Section~\ref{sec:findings} with an emphasis on answering the hypotheses. Finally, we present discussion of our results and provide directions for future work in Section~\ref{sec:conclusion}. 

We end this section by defining key notations to be used throughout this paper. Let $\triangle(X)$ denote the set of all probability distributions on $X$. 
For an integer \( n \), we let \( [n]:= \{1, 2, \ldots, n\} \). For $\lambda \geq 0$, let $\simplex_n:=\setdef{x \in \real_{\geq 0}^n}{\sum_{i \in (n)} x_i = 1}$ be the $(n-1)$-dimensional probability simplex.



==> An Experimental Study on Learning Correlated Equilibrium in Routing Games/survey-ks.tex <==
\subsection{Feedback Survey}
\begin{enumerate}
\item On the scale of 1 to 5 (with 5 being the highest), how did you feel you understood what was happening in each scenario, what you were doing and what you needed to do next?
\item On the scale of 1 to 5 (with 5 being the highest), how often did you check the average star rating before making route choice decisions?
\item When you indeed checked the average star rating, on the scale of 1 to 5 (with 5 being the highest), how much did the average star rating affect your route choice decisions?
\item On the scale of 1 to 5 (with 5 being the highest), how often did you check the histograms before making route choice decisions?
\item When you indeed checked the histograms, on the scale of 1 to 5 (with 5 being the highest), how much did the histograms affect your route choice decisions?
\item How did you make your route choice decisions?
\begin{enumerate}
\item Study the average star rating, histograms as well as the recommendations to come up with a decision.
\item Follow the recommendations as long as the average star rating is above certain value.
\item Always follow the recommendations.
\item Make random choices.
\end{enumerate}
\item If you choose (b) in question 6, what was the threshold value? 
\item What did you like (if any) or dislike (if any) about the experiment interface?
\item Any other comments you might have
\end{enumerate}

==> An Experimental Study on Learning Correlated Equilibrium in Routing Games/tikz_config-ks.tex <==
\usepackage{tikz}
\usepackage{standalone}
\usepackage{pgfplots}
\usetikzlibrary{positioning}
\usetikzlibrary{shapes, arrows.meta, arrows}
\usepackage{relsize}
%
%\tikzset{fontscale/.style = {font=\relsize{#1}}
%    }
%
%\definecolor{nodecolor}{rgb}{255, 255, 255}
%\definecolor{sourcenodecolor}{rgb}{255, 0, 0}
%\definecolor{sinknodecolor}{rgb}{0, 255, 0}

%\tikzset{ dot/.style ={circle, draw, inner sep=2pt},  
%	     supply dot/.style ={circle, draw, inner sep=2pt, fill = sourcenodecolor}, 
%	     demand dot/.style={circle, draw, inner sep=2pt, fill = sinknodecolor},
%              main node/.style={circle,draw,font=\sffamily\bfseries\small, fill=nodecolor, line width = 0.5mm}, 
%              supply node/.style={circle,draw,font=\sffamily\bfseries\small, fill=sourcenodecolor, line width = 0.5mm}, 
%              demand node/.style={circle,draw,font=\sffamily\bfseries\small, fill=sinknodecolor, line width = 0.5mm},
%              edge label/.style={font=\sffamily\small},
%              main edge/.style={thick, auto},
%              directed edge/.style={-Stealth,thick, auto}, 
%              cascading edge/.style={line width=0.75mm, auto},
%              infeasible node/.style={circle,minimum size=0.6cm, inner sep=0pt, draw, fill= red!50}, 
%              feasible node/.style={circle,minimum size=0.6cm, inner sep=0pt, draw, fill= blue!50},
%              face/.style={circle,draw,inner sep=1pt, fill=black}}

% use ``pgfplot '' to plot function in tikz pictures

==> extra-stuff-ks.tex <==
\subsection{Extra Stuff}
We now describe the modifications to the model in \eqref{eq:instant}-\eqref{eq:p flow dynamics-m-general-matrix} to align it with the experimental setup. 
\begin{itemize}
\item Recall from \eqref{eq:instant}-\eqref{eq:p flow dynamics-m-general-matrix}  that matrix $P$ is used in the computation of regret. Since we do not know $P$ a priori, we replace it with the following online estimate for the $s$-th agent:
\begin{equation*}
\hat{P}_{i,j}^{s}= \frac{N(s-1;i,j)}{\sum_{j \in (\nlinks)} N(s-1;i,j)}, \quad i, j \in (\nlinks)
\end{equation*}
where $N(s-1;i,j)$ is the number of times agents $1$ thru $s-1$ choose route $j$ when recommended route $i$. That is, $\hat{P}^{s}$ is constant during session of agent $s$.

\item At the beginning of scenario $k$, participant $\#n$ checks the average review rating $R^{\#n}[k]$ (maximum 5 star rating), combines with the recommended route and the histograms, participant $\#n$ makes his or her route choice decision. Irrespective of participant $\#n$'s decision, the route flow on route $i, i \in (3)$ is given by: 
\begin{equation*}
\label{eq:p flow dynamics-m-general}
\begin{split}
f_i(R^{\#n}[k],\omega[k]) = \pi_i^{\omega[k]} \frac{R^{\#n}[k]}{5} + \sum_{j \in (3)} P^{\#n}_{ji} \pi_j^{\omega[k]} \left(1-\frac{R^{\#n}[k]}{5}\right)
\end{split}
\end{equation*}


\item We mimic the simultaneous routing behavior of multiple participants by incorporating submitted review ratings of all past participants, under the same realized state of nature $\omega[k]$ and the same quantized average review rating $\tilde{R}^{\#n}[k]$ (quantization step = 0.5), when updating the average review rating $R^{\#n}[k+1]$ after participant $\#n$ submitted his or her review rating $r^{\#n}[k]$. Let $\mc R^{\#n}_{\omega[k],\tilde{R}^{\#n}[k]}:=\{r^{\#h}[t] | h \in (n), \omega[t]=\omega[k], \tilde{R}^{\#h}[t]=\tilde{R}^{\#n}[k]\}$, the instantaneous aggregated rating is given by:
\begin{equation*}
\bar{r}^{\#n}[k] := \frac{\sum_{r^{\#h}[t] \in \mc R^{\#n}_{\omega[k],\tilde{R}^{\#n}[k]}} r^{\#h}[t]}{\left|\mc R^{\#n}_{\omega[k],\tilde{R}^{\#n}[k]}\right|}
\end{equation*}
The average review rating of scenario $k+1$ for participant $\#n$ is given by:
\begin{equation*}
R^{\#n}[k+1]=\frac{k}{k+1}R^{\#n}[k]+\frac{1}{k+1}\bar{r}^{\#n}[k]
\end{equation*}
Then, participant $\#n$ will enter scenario $k+1$ with the updated average review rating $R^{\#n}[k+1]$, untill $k=100$ and the experiment session will end for participant $\#n$. 
\end{itemize}


%\subsection{Repeated Game Setting}
%Consider the following repeated game setting. The strategy space of a participant is $\{\mathrm{obey}, \mathrm{do \, not \, obey}\}$. The $\mathrm{do \, not \, obey}$ behavior of the participant is modeled by the row-stochastic matrix $P$ with zeros on the diagonal, where $P_{ij}$ is the fraction of $\mathrm{do \, not \, obey }$ participants who are recommended route $i$ but choose $j$. 
%
%In the experiment study, we use the route choice data from participant $\#1$ up to $\#n-1$ to calculate $P^{\#n}$ for participant $\#n$. For example, $P^{\#n}_{ij} := \frac{\text{total number of times of choosing route j when recommended route i for participants \#1 up to \#n-1}}{\text{total number of times of not following the recommendation when recommended route i for participants \#1 up to \#n-1}}$. 

After making his or her route choice for scenario $k$, participant $\#n$ will then have access to realized actual travel times $\{\ell_i^{\omega[k]}\}_{i \in (3)}$, and be asked to evaluate the quality of the recommendation and submit a rating $r^{\#n}[k]$. 

\ksmargin{move it to later?}
\kscomment{Note that, we set the initial values of average review rating $R^{\#n}[1]$ for all participants $n$ to be 2.5.}

In our theoretical work, the choice of a participant is driven by a notion of regret. To study the relation between instantaneous aggregated average rating and regret, we have to define regret properly. In our theoretical work, the regret model requires knowledge of $P$, which can only be computed using historical data of all previous participants and is inaccessible to the current participants. Based on the available information in our user interface, which consists of actual travel times of all 3 routes, we redefined the individual regret as the difference between the actual travel time of recommended route and fastest route.

After making his or her route choice for scenario $k$, participant $\#n$ will then have access to realized actual travel times $\{\ell_i^{\omega[k]}\}_{i \in (3)}$, and compute the instantaneous regret $m^{\#n}[k]$ as the difference between the travel time associated with the recommended route and the shortest travel time. Similar to the aggregation mechanism of instantaneous aggregated rating, we incorporate instantaneous regrets of all past participants, under the same realized state of nature $\omega[k]$ and the same quantized average review rating $\tilde{R}^{\#n}[k]$ (quantization step = 0.5), when calculating the instantaneous aggregated regret $\bar{m}^{\#n}[k]$. Let $\mc M^{\#n}_{\omega[k],\tilde{R}^{\#n}[k]}:=\{m^{\#h}[t] | h \in (n), \omega[t]=\omega[k], \tilde{R}^{\#h}[t]=\tilde{R}^{\#n}[k]\}$, the instantaneous aggregated regret is given by:
\begin{equation*}
\bar{m}^{\#n}[k] := \frac{\sum_{m^{\#h}[t] \in \mc M^{\#n}_{\omega[k],\tilde{R}^{\#n}[k]}} m^{\#h}[t]}{\left|\mc M^{\#n}_{\omega[k],\tilde{R}^{\#n}[k]}\right|}
\end{equation*}
And the time-averaged aggregated regret is given by:
\begin{equation*}
\tilde{m}^{\#n}[k] := \frac{1}{k} \sum_{t=1}^k \bar{m}^{\#n}[t]
\end{equation*}
